Performance Analysis of AFDM Transceiver Under Practical IQ Imbalance

This paper investigates the impact of in-phase/quadrature (IQ) imbalance on signal detection in affine frequency-division multiplexing (AFDM) systems over doubly dispersive Rayleigh fading channels. The bit error rate (BER) performance of AFDM under various IQ mismatch conditions is evaluated and compared with that of an ideal transceiver. Simulation results show that, under ideal conditions, BER decreases rapidly with increasing signal-to-noise ratio (SNR). However, IQ imbalance introduces image interference that spreads across the affine domain, causing significant performance degradation. The results further highlight the impact of practical IQ imbalance on AFDM systems across different quadrature amplitude modulation (QAM) orders, channel scenarios, and comparisons with orthogonal frequency-division multiplexing (OFDM) and orthogonal time frequency space (OTFS) systems. In particular, higher-order QAM performance degrades significantly, indicating the need for IQ imbalance compensation techniques or impairment-aware detection algorithms to ensure robust operation in practical AFDM systems.

==> NEW_VALUES.tex <==
snr value
0    0.198577008928571
2    0.153926339285714
4    0.112773437500000
6    0.076469866071429
8   0.046910714285714
10    0.026685267857143
12    0.013639508928571
 14   0.006352678571429
16    0.002776785714286
 18   0.001121651785714
 20   0.0004843750000000000
 22   0.0001953125000000000
24   0.00008147321428571429
26    0.00002343750000000000
28    0.00001450892857142857
30    0.000004464285714285715

